S2-Track: A Simple yet Strong Approach for End-to-End 3D Multi-Object Tracking

3D multiple object tracking (MOT) plays a crucial role in autonomous driving perception. Recent end-to-end query-based trackers simultaneously detect and track objects, which have shown promising potential for the 3D MOT task. However, existing methods are still in the early stages of development and lack systematic improvements, failing to track objects in certain complex scenarios, like occlusions and the small size of target object's situations. In this paper, we first summarize the current end-to-end 3D MOT framework by decomposing it into three constituent parts: query initialization, query propagation, and query matching. Then we propose corresponding improvements, which lead to a strong yet simple tracker: S2-Track. Specifically, for query initialization, we present 2D-Prompted Query Initialization, which leverages predicted 2D object and depth information to prompt an initial estimate of the object's 3D location. For query propagation, we introduce an Uncertainty-aware Probabilistic Decoder to capture the uncertainty of complex environment in object prediction with probabilistic attention. For query matching, we propose a Hierarchical Query Denoising strategy to enhance training robustness and convergence. As a result, our S2-Track achieves state-of-the-art performance on nuScenes benchmark, i.e., 66.3% AMOTA on test split, surpassing the previous best end-to-end solution by a significant margin of 8.9% AMOTA. We achieve 1st place on the nuScenes tracking task leaderboard.

==> latex/fig/uncertainty.tex <==
\begin{figure}[t]
  \centering
   \vspace{-1pt}
  \includegraphics[width=1\linewidth]{pics/uncertainty.pdf}
  \vspace{-15pt}
  \caption{\textbf{The uncertainty analysis}. \name{} consistently outperforms state-of-the-art tracker PF-Track~\cite{pang2023PFtrack} under different uncertainty situations, especially under severe occlusions and small object size settings.
  }
  \label{fig:uncertainty}
   \vspace{-5pt}
\end{figure}
